Beyond Parameter Aggregation: Semantic Consensus for Federated Fine-Tuning of LLMs

Federated fine-tuning of large language models is commonly formulated as a parameter aggregation problem. However, even parameter-efficient methods require transmitting large collections of trainable weights, assume aligned architectures, and rely on white-box access to model parameters. As model sizes continue to grow and deployments become increasingly heterogeneous, these assumptions become progressively misaligned with practical constraints. We consider an alternative formulation in which collaboration is mediated through model behavior rather than parameters. Clients fine-tune local models on private data and exchange generated outputs on a shared, public prompt set. The server maps these outputs into a semantic representation space, forms a per-prompt semantic consensus, and returns pseudo-labels for further local fine-tuning. This formulation fundamentally changes the communication scaling of federated LLM fine-tuning. The amount of information exchanged depends only on the public prompt budget and the size of the communicated behaviors, independent of model size. As a consequence, the protocol naturally accommodates heterogeneous architectures and applies directly to open-ended text generation. We present a theoretical analysis and empirical results demonstrating that this approach can match strong federated fine-tuning baselines while substantially reducing communication by orders of magnitude (e.g., analytically by a factor of $1006$ for Llama3.1-405B), as well as reductions in runtime and energy consumption. These results suggest that, for generative foundation models, behavior-level consensus provides a more appropriate abstraction for federated adaptation than parameter aggregation.

==> preamble.tex <==
\RequirePackage{amsthm, amsmath, amssymb}
%\usepackage{algorithm, algpseudocode}
\usepackage{fancyvrb}

\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0.0,0,0.75}
\definecolor{verdigreen}{rgb}{0.0, 0.5, 0.0}

%\usepackage{hyperref}
\usepackage[colorlinks]{hyperref}
%\PassOptionsToPackage{hidelinks=false,colorlinks=true, citecolor=darkblue, urlcolor=darkblue,linkcolor=darkblue}{hyperref}    
\hypersetup{
  urlcolor     = darkblue, %Colour for external hyperlinks
  linkcolor    = darkblue, %Colour of internal links
  citecolor   = darkblue, %Colour of citations
  pdftitle=\ourtitle, 
  pdfauthor=anonymous,
  breaklinks
}
\usepackage{makecell}

\usepackage{url}
\usepackage{multirow}
\usepackage[dvipsnames]{xcolor}
\def\UrlFont{\rm}  
\usepackage{natbib} 
\usepackage{caption} 
%\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{diagbox}
\usepackage{float}
\usepackage{mathtools}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xfrac}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{bbm}
%\usepackage[caption=false]{subfig}
%\usepackage{eufrak}
\usepackage{dsfont}
\usepackage[ruled, vlined, nofillcomment, linesnumbered, noline, norelsize]{algorithm2e}
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\usepackage[export]{adjustbox}
\usepackage{amsthm}   
\usepackage{tikz}
\usepackage{verbatim}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{soul} % use this (many fancier options)
\usepackage{subfigure}
\usepackage{thm-restate}

% Packages
\usepackage{latexsym}
\usepackage{makecell} 
%\usepackage[ruled, vlined, nofillcomment, linesnumbered, noline, noend]{algorithm2e}
%used for stricking out text
%\usepackage[normalem]{ulem}

\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}

\DeclareMathSymbol{\Lt}{3}{matha}{"CE}
\DeclareMathSymbol{\Gt}{3}{matha}{"CF}
